Theorie des longitudinalen Atomstrahl-Spinechos und paritaetsverletzende Berry-Phasen in Atomen

We present a nonrelativistic theory for the quantum mechanical description of longitudinal atomic beam spin echo experiments, where a beam of neutral atoms is subjected to static electric and magnetic fields. The atomic wave function is the solution of a matrix-valued Schroedinger equation and can be written as superposition of local (atomic) eigenstates of the potential matrix. The position- and time-dependent amplitude function of each eigenstate represents an atomic wave packet and can be calculated in a series expansion with a master formula that we derive. The zeroth order of this series expansion describes the adiabatic limit, whereas the higher order contributions contain the mixing of the eigenstates and the corresponding amplitude functions. We give a tutorial for the theoretical description of longitudinal atomic beam spin echo experiments and for the so-called Fahrplan model, which is a visualisation tool for the propagation of wave packets of different atomic eigenstates. As an example for the application of our theory, we study parity violating geometric (Berry-)phases. In this context, we define geometric flux densities, which for certain field configurations can be used to illustrate geometric phases in a vector diagram. Considering an example with a specific field configuration, we prove the existence of a parity violating geometric phase.

==> Kapitel09.tex <==

\FloatBarrier

%********************************************************************************************
%============================================================================================
\chapter{Untersuchung P-verletzender Effekte mit Hilfe geometrischer Phasen}\label{s9:geom.Phasen}
%============================================================================================
%********************************************************************************************

Die ursprüngliche Idee für den Nachweis paritätsverletzender Effekte in leichten Atomen basiert
auf dem mehrmaligen An- und Ausschalten eines schwachen elektrischen Feldes, in dem sich das betrachtete,
metastabile Atom (Wasserstoff oder Deuterium) ruht. Hierdurch erfährt es sukzessive Drehnungen der Polarisation,
die zum Teil paritätsverletzend sind (siehe ...). Der Effekt konnte theoretisch auf einen P-verletzenden Anteil von
5\% in der gesamten Polarisationsdrehung maximiert werden, wobei man hierfür etwa $10^6$ hintereinander
geschaltete elektrische Felder benötigen würde (siehe ...).

\begin{figure}[!hb]
  \centering
  \includegraphics[width=10cm]{Figures/PV-ABSE-Problem}
  \caption{Schematischer Fahrplan bei Verwendung multipler, hintereinandergeschalteter elektrischer Felder}
  \label{f9:PV-ABSE-Problem}
\end{figure}
Neben dem Problem, experimentell eine derart große Anzahl von kurzen und schwachen elektrischen Felder zu
realisieren, gibt es bei der Verwendung des longitudinalen Spinechos noch eine weitere Schwierigkeit.
Betrachten wir hierzu als Beispiel ein einfaches zwei-Zustands-System und nehmen an, dass in jedem elektrischen
Feld ein Teil des Zustands $\ket{1}$ in den Zustand $\ket{2}$ übergeht. Starten wir mit einem Wellenpaket
im Zustand $\ket1$, siehe Abb. \ref{f9:PV-ABSE-Problem}, 
so wird im ersten $\mc E$-Feld ein (wenn auch noch so kleines) Wellenpaket des Zustands
$\ket2$ produziert, dessen Schwerpunktsgeschwindigkeit im feldfreien Raum (je nach Energiedifferenz)
von der des Pakets des Zustands $\ket1$ abweicht.
Beide Pakete treffen dann zu leicht unterschiedlichen Zeiten beim zweiten $\mc E$-Feld ein und spalten dort
wieder ein neues Wellenpaket des jeweils anderen Zustands ab.
Wie man sieht, überlagern sich die Wellenpakete zum gleichen Zustand nur teilweise. Für einen maximalen,
P-Verletzenden Effekt ist es nach der ursprünglichen Idee dagegen unbedingt notwendig, ein ausgeprägtes
Wellenpaket zu jedem Zustand zu haben und diese dann zur Interferenz zu bringen.
In Abb. \ref{f9:PV-ABSE-Problem} erkennt man jedoch, dass viele Wellenpakete des gleichen Zustands
in kurzen Zeitabständen beim Detektor eintreffen würden, begründet durch die mehrfache Aufspaltung
der Zustände in den elektrischen Feldern. Dieses Problem bestand bei der in früheren
Arbeiten verwendeten idealisierten Betrachtung eines Atoms in Ruhe in einem zeitlich veränderlichen elektrischen Feld 
nicht.

\section{P-Verletzung in geometrischen Phasenfaktoren}

\newcommand{\phiw}{\phi\supt{WKB}}
\newcommand{\phig}{\phi\supt{geom.}}
\newcommand{\phiz}{\phi\supt{Zerfall}}
\newcommand{\phia}{\phi\supt{Amp.}}

Wir bauen hier auf den Grundlagen aus Kapitel \ref{s6:Formalismus} auf, wo wir die matrixwertige Schrödinger-Gleichung
gelöst haben. Wir erinnern uns nun an den dort gewählten Phasenwinkel $\phi_\alpha(Z,t)$, der in dem Ansatz für die
Komponentenwellenfunktionen
\begin{align}\label{e9:Komp.Psi}
  \Psi_\alpha(Z,t) = \e^{\I\phi_\alpha(Z,t)}A_\alpha(Z,t)
\end{align}
des Gesamtzustands
\begin{align}\label{e9:Ges.Psi}
  \ket{\Psi(Z,t)} = \sum_\alpha\Psi_\alpha(Z,t)\rket{\alpha(Z)}
\end{align}
verwendet wurde. Es war, nach Gl. (\ref{e6:PW}),
\begin{align}\label{e9:PW}
  \phi_\alpha(Z,t) = \phiw_\alpha(Z,t) + \phig_\alpha(Z,t) + \phiz_\alpha(Z,t) + \phia_\alpha(Z,t)\ ,
\end{align}
mit dem WKB-Anteil
\begin{align}\label{e9:PW.WKB}
  \phiw_\alpha(Z,t) &= -\frac{\bar k^2_\alpha}{2M}t + \int_{Z_0}^Z\d Z'\ k_\alpha(Z')\ ,
\end{align}
dem geometrischen Anteil
\begin{align}\label{e9:PW.geom}
  \phig_\alpha(Z,t) &= \I\int_{u_\alpha(Z,t)}^Z\d Z'\ \lrbra{\alpha(Z')}\del_{Z'}\rket{\alpha(Z')}\ ,
\end{align}
dem Zerfalls-Anteil
\begin{align}\label{e9:PW.Zerfall}
  \phiz_\alpha(Z,t) &= -\frac\I2\int_{u_\alpha(Z,t)}^Z\d Z'\ \frac{M\Gamma_\alpha(Z')}{k_\alpha(Z')}
\end{align}
und dem Anteil für die Amplitudenkorrektur,
\begin{align}\label{e9:PW.Amp}
  \phia_\alpha(Z,t) &= -\I\ln\kappa_\alpha(Z,t)\ .
\end{align}
Für die Definitionen der verwendeten Größen $\bar k_\alpha$, $k_\alpha(Z)$, $u_\alpha(Z,t)$ und $\kappa_\alpha(Z,t)$
verweisen wir auf Kapitel \ref{s6:SG}.

Wir interessieren uns hier besonders für den geometrischen Anteil (\ref{e9:PW.geom}) und wollen im Folgenden
untersuchen, ob und wie stark P-verletzende Beiträge zu dieser geometrischen Phase beitragen. Gelingt es, bereits im 
adiabatischen Grenzfall durch geschickte Wahl der elektrischen und magnetischen Felder den P-verletzenden Anteil in
der geometrischen Phase auf einen messbaren Effekt zu maximieren, so könnte man sich die äußerst aufwendige numerische
Berechnung der ersten Ordnung der Entwicklung im Integraloperator $\hat{\umc K}$ ersparen. Solange die experimentellen
Parameter so gewählt sind, dass die adiabatische Näherung eine gute Näherung darstellt, können wir numerisch sehr genau 
rechnen. Ist die adiabatische Näherung nicht mehr erfüllt, so werden auch höhere Ordnungen der Entwicklung in
$\hat{\umc K}$ zu berücksichtigen sein und es ist (zum jetzigen Zeitpunkt) noch unklar, ob und mit welcher Genauigkeit
die Berechnung der komplizierten Integrale, die u.a. komplexe Phasenfaktor enthalten, zu bewerkstelligen wäre.
Diese offene Frage, die aus Zeitgründen in der vorliegenden Arbeit nicht beantwortet werden kann, muss in zukünftigen
Arbeiten untersucht werden.

Wir betrachten hier also nur den adiabatischen Grenfall, d.h. wir setzen
\begin{align}\label{e9:Psi.ad}
  \Psi_\alpha(Z,t) \approx \hat\chi_\alpha\e^{\phi_\alpha(Z,t)}\vph(\zeta_\alpha(Z)-\tau(t))\rket{\alpha(Z)}\ .
\end{align}
Die Koeffizienten $\hat\chi_\alpha$ sind wie üblich aus der Polarisation den Anfangszustands zu bestimmen. Die Einhüllende
$\vph(\zeta)$ (das Anfangswellenpaket) kann für alle Komponenten o.B.d.A. gleich gewählt werden.

Kommen wir nun zur P-Verletzung. Wie in Anhang \ref{sB:Vorspiel} dargestellt, gibt es einen P-verletzenden Beitrag
in der ortsunabhängigen, freien Massenmatrix $\uop M_0$. Die Matrixelemente des entsprechenden Hamiltonoperators
$H\PV$ sind in (\ref{eB:HPV}) angegeben, wobei es einen spinunabhängigen Anteil proportional zum paritätsverletzenden 
Parameter $\delta_1$ und einen vom Gesamt- und Kernspin abhängigen Anteil proportional zu $\delta_2$ gibt. Die
Parameter $\delta_{1,2}$ haben extrem kleine numerische Werte, $\delta_{1,2} = 10^{-13}..10^{-12}$ und treten in
der Massenmatrix stets in Verbindung mit der Lamb-Shift $\mc S$ auf. Die Matrixelemente des P-Verletzenden Anteils
$\uop M\PV$ sind also ebenfalls extrem klein im Vergleich zu den übrigen Matrixelementen der freien Massenmatrix.
Wir fassen den Anteil $\uop M\PV$ deshalb als Störung auf, wobei wir die $\delta_{1,2}$ als Störparameter verwenden.
Wir schreiben die gesamte Massenmatrix als
\begin{align}\label{e9:MMPV}
  \uop M(Z) = \uop{\hat M}(Z) + \delta_1\uop M\PV^{(1)} + \delta_2\uop M\PV^{(2)}\ ,
\end{align}
wobei nun die Matrixelemente der so definierten Matrizen $\uop M^{(1,2)}$ - da proportional zur Lamb-Shift - 
nicht mehr klein gegen die Matrixelemente von $\uop{\hat M}(Z)$ sind. 

Um die Formeln für die Störungstheorie leichter anwenden zu können schreiben wir symbolisch 
$\delta\uop M\PV$ für $\delta_i\uop M\PV^{(i)}$, $i=1,2$. In der Störungsentwicklung des Zustands

\begin{align}\label{e9:MPV}
  \delta\uop M\PV = \delta_1\uop M\PV^{(1)} + \delta_2\uop M\PV^{(2)}\ ,
\end{align}
und weiter
\begin{align}
  \rket{\alpha(Z,\delta)} &= \rket{\alpha_0(Z)} + \delta\rket{\alpha_1(Z)} + \OO(\delta^2)\ ,\\
  \lrbra{\alpha(Z,\delta)} &= \mc N_\alpha(Z,\delta)\kle{\lrbra{\alpha_0(Z)} + \delta\lrbra{\alpha_1(Z)} + \OO(\delta^2)}\ .
\end{align}
Dabei sind die mit Null indizierten Zustände die Eigenzustände der P-erhaltenden Massenmatrix $\uop{\hat M}(Z)$.
Auf der linken Seite stehen die jeweils gestörten Eigenvektoren der Massenmatrix, die wir im Prinzip
in allen Formeln des Matrixformalismus zu verwenden haben. Wir schreiben deshalb im Folgenden die Abhängigkeit
von den P-verletzenden Parametern (bzw. symbolisch für $\delta$) explizit aus, d.h. es ist
\begin{align}
  \rket{\alpha(Z)} \equiv \rket{\alpha(Z,\delta)} \equiv \rket{\alpha(Z,\delta_1,\delta_2)}\ .
\end{align}
Wir werden je nach Bedarf alle drei Schreibweisen verwenden, um die Übersichtlichkeit so groß wie möglich zu halten.

Die störungstheoretische Berechnung der Eigenvektoren der gesamten Massenmatrix $\uop M(Z)$ erfolgt mit den in
Anhang \ref{sA:StoeRe} angegebenen Methoden. In Gl. (\ref{eA:Projektorentwicklung}) ist die Störungsentwicklung des
Quasiprojektors
\begin{align}\label{e9:QPro}
  \Pro_\alpha(Z,\delta) &= \rket{\alpha(Z,\delta)}\lrbra{\alpha(Z,\delta)}
\end{align}
angegeben. Mit ihm berechnen sich die gestörten Zustände nach Gl. (\ref{eA:Zustandsentwicklung}) aus den ungestörten 
Zuständen durch einfache Projektion:
\begin{subequations}
\begin{align}
  \rket{\alpha(Z,\delta)}  &= \Pro_\alpha(Z,\delta)\rket{\alpha_0(Z)}\ ,\\
  \lrbra{\alpha(Z,\delta)} &= \mc N_\alpha(Z,\delta)\lrbra{\alpha_0(Z)}\Pro_\alpha(Z,\delta)\ ,\\
  \mc N_\alpha(Z,\delta) &= \kle{\Spur(\Pro_\alpha(Z,\delta)\Pro_\alpha^{(0)}(Z))}^{-1}\ .
\end{align}
\end{subequations}
Dabei ist
\begin{align}
  \Pro_\alpha^{(0)}(Z) = \rket{\alpha_0(Z)}\lrbra{\alpha_0(Z)}
\end{align}
der Quasiprojektor der ungestörten (P-erhaltenden) Eigenzustände der Massenmatrix.

Aus der Formel (\ref{eA:Projektorentwicklung}) aus Anhang \ref{sA:StoeRe} lesen wir die Entwicklung des Quasiprojektors
wie folgt ab:
\begin{align}\label{e9:QPro1}
  \Pro_\alpha(Z,\delta) &= \Pro_\alpha^{(0)}(Z) + \delta\sum_{\beta\neq\alpha}
    \frac{\Pro_\alpha^{(0)}(Z)\uop M\PV\Pro_\beta^{(0)}(Z) + \Pro_\beta^{(0)}(Z)\uop M\PV\Pro_\alpha^{(0)}(Z)}{E_\alpha^{(0)}(Z) - E_\beta^{(0)}(Z)} + \OO(\delta^2)\ .
\end{align}
Aus (\ref{eA:Norm}) folgt weiterhin
\begin{align}\label{e9:Norm}
  \mc N_\alpha(Z,\delta) = 1 + \OO(\delta^2)\ .
\end{align}
Die Korrekturen zur Energie sind zwar auch im Prinzip in der Ordnung $\OO(\delta)$ vorhanden, allerdings wurde bereits in
\cite{BoBrNa95} (Abschnitt 3.4) gezeigt, dass aus Gründen der Zeitumkehrinvarianz unter den hier gültigen 
Voraussetzungen\footnote{Die Eigenwerte müssen in einem Bereich um $\delta_i=0$, der $\delta_i$ und $-\delta_i$
einschließt ($i=1,2$), nichtentartet sein.} die Energieverschiebungen nur von Geraden Potenzen der $\delta_i$-Parameter 
abhängen. Somit gilt also für die gestörten Energien
\begin{align}\label{e9:Energie}
  E_\alpha(Z,\delta) = E^{(0)}_\alpha(Z) + \OO(\delta^2)\ .
\end{align}
Beiträge der Ordnung $\OO(\delta^2)$ werden aufgrund der geringen Größe der P-verletzenden Beiträge konsequent vernachlässigt.

Mit der Formel (\ref{e9:QPro1}) für den Quasiprojektor und der Normierung aus (\ref{e9:Norm}) erhalten wir
für die Korrekturbeiträge der linken und rechte Eigenzustände schließlich
\begin{subequations}
\begin{align}\label{e9:R.Ket.1}
  \delta\rket{\alpha_1(Z)} &= \delta\sum_{\beta\neq\alpha}
      \frac{\Pro_\beta^{(0)}(Z)\uop M\PV\rket{\alpha_0(Z)}}{E^{(0)}_\beta(Z)-E^{(0)}_\alpha(Z)}\ ,\\ \label{e9:L.Bra.1}
  \delta\lrbra{\alpha_1(Z)} &= \delta\sum_{\beta\neq\alpha}
      \frac{\lrbra{\alpha_0(Z)}\uop M\PV\Pro_\beta^{(0)}(Z)}{E^{(0)}_\beta(Z)-E^{(0)}_\alpha(Z)}\ .
\end{align}
\end{subequations}

Dies können wir nun auf die geometrische Phase aus (\ref{e9:PW.geom}) anwenden. Wir betrachten zunächst nur den Integranden,
d.h.
\begin{align}
  \begin{split}
  &~\lrbra{\alpha(Z,\delta)}\del_Z\rket{\alpha(Z,\delta)}\\
  =&~\lrbra{\alpha_0(Z)}\del_Z\rket{\alpha_0(Z)} 
    + \delta\kle{\lrbra{\alpha_0(Z)}\del_Z\rket{\alpha_1(Z)} + \lrbra{\alpha_1(Z)}\del_Z\rket{\alpha_0(Z)}}
    + \OO(\delta^2)\ .
  \end{split}
\end{align}
Offensichtlich gilt $\lrbra{\alpha_0(Z)}\alpha_1(Z)) = \lrbra{\alpha_1(Z)}\alpha_2(Z)) = 0$, also folgt aus der
Ortsableitung dieser Ausdrücke
\begin{align}
  \begin{split}
    \lrbra{\alpha_0(Z)}\overset{\leftharpoonup}\del_Z\rket{\alpha_1(Z)} &= 
      -\lrbra{\alpha_0(Z)}\del_Z\rket{\alpha_1(Z)}\ ,\\
    \lrbra{\alpha_1(Z)}\overset{\leftharpoonup}\del_Z\rket{\alpha_0(Z)} &= 
      -\lrbra{\alpha_1(Z)}\del_Z\rket{\alpha_0(Z)}
  \end{split}
\end{align}
und somit
\begin{align}\label{e9:D10LR}
  \begin{split}
  &~\lrbra{\alpha(Z,\delta)}\del_Z\rket{\alpha(Z,\delta)}\\
  =&~\lrbra{\alpha_0(Z)}\del_Z\rket{\alpha_0(Z)} 
    + \delta\kle{\lrbra{\alpha_1(Z)}\del_Z\rket{\alpha_0(Z)} -
        \lrbra{\alpha_0(Z)}\overset{\leftharpoonup}\del_Z\rket{\alpha_1(Z)}}
    + \OO(\delta^2)\ .
  \end{split}
\end{align}
und weiter
\begin{align}\label{e9:PV.MatElem.1}
  \begin{split}
     &~\lrbra{\alpha(Z,\delta)}\del_Z\rket{\alpha(Z,\delta)}\\
    =&~\lrbra{\alpha_0(Z)}\del_Z\rket{\alpha_0(Z)} 
      + \delta\sum_{\beta\neq\alpha}\frac{1}{E^{(0)}_\alpha(Z)-E^{(0)}_\beta(Z)}\\
    \times&\kle{
      \lrbra{\alpha_0(Z)}\uop M\PV\rket{\beta_0(Z)}\lrbra{\beta_0(Z)}\del_Z\rket{\alpha_0(Z)}
    - \lrbra{\alpha_0(Z)}\overset{\leftharpoonup}\del_Z\rket{\beta_0(Z)}\lrbra{\beta_0(Z)}\uop M\PV\rket{\alpha_0(Z)}}
  \end{split}
\end{align}
Wir können nun wieder die in Kapitel \ref{s6:Formalismus} definierten Ableitungsmatrizen
\begin{align}
  \uop D^{(1)}_{\beta\alpha}(Z) = \lrbra{\beta_0(Z)}\del_Z\rket{\alpha_0(Z)}
\end{align}
verwenden, wobei wir von jetzt an vereinbaren, dass sich alle Matrixdarstellungen mit griechischen Indizes auf die
P-erhaltenden, ungestörten Eigenvektoren $\rket{\alpha_0(Z)}$ der Massenmatrix $\uop{\hat M}(Z)$ beziehen. Aus der Orthonormalität dieser Zustände erhalten wir analog zu (\ref{e9:D10LR})
\begin{align}\label{e9:D00LR}
  \begin{split}
    \lrbra{\beta_0(Z)}\overset{\leftharpoonup}\del_Z\rket{\alpha_0(Z)} &= 
      -\lrbra{\beta_0(Z)}\del_Z\rket{\alpha_0(Z)}\ ,\\
    \lrbra{\alpha_0(Z)}\overset{\leftharpoonup}\del_Z\rket{\beta_0(Z)} &= 
      -\lrbra{\alpha_0(Z)}\del_Z\rket{\beta_0(Z)}\ .
  \end{split}
\end{align}
Damit können wir in (\ref{e9:PV.MatElem.1}) die nach links wirkende Ableitung ebenfalls mit der Ableitungsmatrix schreiben 
und erhalten
\begin{align}\label{e9:PV.Geom.Integrand}\hspace{-3mm}
    \lrbra{\alpha(Z,\delta)}\del_Z\rket{\alpha(Z,\delta)} &= \uop D^{(1)}_{\alpha\alpha}(Z)
      + \delta\sum_{\beta\neq\alpha}\frac{\klr{\uop M\PV}_{\alpha\beta}\uop D^{(1)}_{\beta\alpha}(Z)
        + \uop D^{(1)}_{\alpha\beta}(Z)\klr{\uop M\PV}_{\beta\alpha}}{E^{(0)}_\alpha(Z)-E^{(0)}_\beta(Z)}
\end{align}

Wir wollen nun studieren, welche Eigenschaften der P-verletzende Beitrag zum Ableitungsmatrixelement hat. Dazu definieren
wir die Hilfsmatrix
\begin{align}
  \uop{\tilde D}_{\alpha\beta}^{(1)} := \klr{1-\delta_{\alpha\beta}}\frac{\uop D^{(1)}_{\alpha\beta}(Z)}{
    E_\alpha^{(0)}(Z)-E_\beta^{(0)}(Z) + \delta_{\alpha\beta}} =
    \begin{cases}
      0 & (\alpha = \beta)\\
      \frac{\uop D^{(1)}_{\alpha\beta}(Z)}{E_\alpha^{(0)}(Z)-E_\beta^{(0)}(Z)} & (\alpha\neq \beta)
    \end{cases}
\end{align}
und schreiben damit kurz unter Verwendung des Kommutators $\kle{A,B} = AB-BA$
\begin{align}
  \lrbra{\alpha(Z,\delta)}\del_Z\rket{\alpha(Z,\delta)} &= \uop D^{(1)}_{\alpha\alpha}(Z)
  + \delta \lrbra{\alpha_0(Z)}\kle{\uop{\tilde D}^{(1)},\uop M\PV}\rket{\alpha_0(Z)}\ .
\end{align}
Die Eigenschaften dieses Kommutators hängen von den Eigenschaften der Ableitungsmatrix ab, die wir nun untersuchen wollen.
Hierfür müssen wir die linken und rechten Eigenzustände genauer betrachten.

Nehmen wir nun an, die Eigenvektoren hängen nur implizit über einen $n$-dimensionalen Vektor von Parametern $\v R(Z)$
von der Ortskoordinate ab (z.B. von den elektrischen und magnetischen Feldern, d.h. $n=6$ und
$\v R(Z) = (\v{\mc E}(Z),\v{\mc B}(Z))\TP$). Dann ist
\begin{align}
  \uop D^{(1)}_{\alpha\beta}(Z) = \sum_{i=1}^n\lrbra{\alpha(\v R)}\ddp{}{R_i}\rket{\beta(\v R)}\dd{R_i(Z)}{Z}
  = \lrbra{\alpha(\v R)}\v\nab_{\v R}\rket{\beta(\v R)}\cdot\dd{\v R(Z)}{Z}
\end{align}
Wir betrachten nun geschlossene Kurven $\mc C$ im Parameterraum, 
die mit der Ortsvariable $Z$ parametrisiert sind. Wir definieren nun
\begin{align}
  \gamma_{\alpha\beta}(\mc C) := \I\int_{\mc C}\uop D^{(1)}_{\alpha\beta}(Z')\d Z'\ .
\end{align}
Das Diagonalelement $\gamma_{\alpha\alpha}(\mc C)$ kann als Differenz der in (\ref{e9:PW.geom})
definierten, geometrischen Phasenwinkel geschrieben werden:
\begin{align}
  \gamma_{\alpha\alpha}(\mc C) = \phig_\alpha(Z_1,t) - \phig_\alpha(Z_0,t)\ .
\end{align}
Hier sind $Z_0$ und $Z_1$ die Parameter für den Anfangs- und Endpunkt der Kurve $\mc C$. Für große Zeiten $t$ wird die
in $\phig_\alpha(Z_0,t)$ vorkommende Integralgrenze $u_\alpha(Z_0,t)$ sicherlich kleiner als $Z_0$. Der Kurventeil
für Parameter kleiner als $Z_0$ soll (nach Voraussetzung) keine Fläche im Parameterraum mehr umschreiben, so die geometrische
Phase für dieses Kurventeil verschwindet. Für genügend große Zeiten $t$ sollte also stets 
$\gamma_{\alpha\alpha}(\mc C) = \phig_\alpha(Z_1,t)$ gelten.

Betrachten wir nun wieder auch nichtdiagonale Komponenten $\gamma_{\alpha\beta}(\mc C)$. Es ist
\begin{align}
  \gamma_{\alpha\beta}(\mc C) = \oint_{\mc C = \del S}\lrbra{\alpha(\v R)}\v\nab_{\v R}\rket{\beta(\v R)}\cdot\d\v R\ .
\end{align}
Im Rahmen der mathematischen Theorie der Differentialformen kann man den Integranden als 1-Form auffassen, d.h.
wir betrachten eine 1-Form
\begin{align}
  \omega = \lrbra{\alpha(\v R)}d\rket{\beta(\v R)}\ ,
\end{align}
wobei der Operator $d$ als äußere Ableitung bezeichnet wird. In unserem Fall ist
\begin{align}
  d = \sum_{i=1}^n \d R_i \ddp{}{R_i}\ .
\end{align}
Wendet man nun den verallgemeinerten Stokesschen Satz an, dann folgt
\begin{align}
  \oint_{\mc C=\del S}\omega = \iint_S d\omega\ ,
\end{align}
wobei $S$ eine von $\mc C$ umrandete, 
beliebige Fläche im Parameterraum sei. Die Berechnung von $d\omega$ gelingt mit Hilfe des äußeren Produkts 
$\wedge$, auch Keilprodukt genannt. Es folgt
\begin{align}
  \begin{split}
    d\omega &= \sum_{i,j=1}^n \ddp{}{R_i} \lrbra{\alpha(\v R)}\ddp{}{R_j}\rket{\beta(\v R)} \d R_i\wedge\d R_j\\
    &= \sum_{1\leq i<j\leq n}  \lrbra{\alpha(\v R)}\overset{\leftharpoonup}\del_i\overset{\rightharpoonup}\del_j - \overset{\leftharpoonup}\del_j\overset{\rightharpoonup}\del_i\rket{\beta(\v R)} \d R_i\wedge\d R_j\ ,
  \end{split}
\end{align}
wobei wir hier die abkürzende Schreibweise
\begin{align}
  \del_i \equiv \ddp{}{R_i}
\end{align}
verwendet haben. Wir haben hier weiter die Antisymmetrie des äußeren Produkts verwendet, d.h.
\begin{align}
  \d R_i\wedge\d R_j = - \d R_j\wedge\d R_i\ .
\end{align}

